Adversarial Attacks on Monocular Pose Estimation

Advances in deep learning have resulted in steady progress in computer vision with improved accuracy on tasks such as object detection and semantic segmentation. Nevertheless, deep neural networks are vulnerable to adversarial attacks, thus presenting a challenge in reliable deployment. Two of the prominent tasks in 3D scene-understanding for robotics and advanced drive assistance systems are monocular depth and pose estimation, often learned together in an unsupervised manner. While studies evaluating the impact of adversarial attacks on monocular depth estimation exist, a systematic demonstration and analysis of adversarial perturbations against pose estimation are lacking. We show how additive imperceptible perturbations can not only change predictions to increase the trajectory drift but also catastrophically alter its geometry. We also study the relation between adversarial perturbations targeting monocular depth and pose estimation networks, as well as the transferability of perturbations to other networks with different architectures and losses. Our experiments show how the generated perturbations lead to notable errors in relative rotation and translation predictions and elucidate vulnerabilities of the networks.

==> TODO.tex <==
%TODO:

- EMPHASISE LOSS IS DUE TO SELF-SUPERVISED.** EMPHASISED SSL IN GENERAL BECAUSE THIS IS WHY DEPTH IS NEEDED **
- EMPHASISE POSE IMPORTANCE IN GENERAL TO SLAM**
- EMPHASISE THAT IN THIS ATTACK, YOU NO LONGER NEED GT TARGETS. **
- ORB-SLAM EXPTS **
- CHECK TRANSFERABILITY ON EPS 0.25, 0.5, 8, AND WITH MD2 MODEL AND OTHER MODELS. **
- CHECK WITH A SUPERVISED POSE MODEL **NOTDOING
- RUN ORB-SLAM ON GAUSSIAN BLUR, DEPTH, AND POSE EXAMPLES. RUN POSE NET ON GAUSSIAN BLUR. **
- REPLACE SELF-SUPERVISED WITH UNSUPERVISED**
- REMOVE FLIPPED ORDER FROM EVERYWHERE**
- CLARIFY THAT WE ONLY LOOK AT DRIVING SCENARIOS (IN INTRO PERHAPS) - NOT NEEDED AS WE DON"T TALK OF FORWARD MOTION BIAS **
- MAKE SURE WHEN SPECIFYING WHICH IMAGE IS SAVED THAT IT WON'T CONFUSE **
- CHECK REFERENCES (ARNAV) **

==> summaries.tex <==
\section{Summaries}
\subsection{SC-Depth}

\subsubsection{Motivation}
Predictions in self-supervised SfM have per-frame scale ambiguity. This is disadvantageous for application to SLAM. So they seek to introduce scale-consistency.

Additionally, they discover a motion mask to remove pixels that violate the static-scene assumption, using the scale-consistency computation, so there is no additional computational overhead. MD2 masks out objects having same velocity as object, but cannot handle other object motions.

\subsubsection{Aims/Contributions}
\begin{itemize}
    \item Propose geometric consistency loss ($L_G$)
    \item Propose self-discovered mask to automatically localize moving objects (since static scene is assumed)
    \item Show efficacy of each component on KITTI and NYUv2 (for depth?)
    \item Have scale consistent prediction due to $L_G$
    \item Using said scale-consistent prediction, they integrate monocular networks into ORB-SLAM.
    \item This pseudo-rgbd slam shows good results on KITTI, generalizes to KAIST. 
    \item This system can start tracking from any frame without latency, has better tracking, and allows for dense 3d reconstruction.
\end{itemize}

\subsubsection{Method}
\begin{itemize}
    \item Unlike MD2, both source(b) and reference frame(a) are passed through depth network, instead of just "a". $D_a$ and $D_b$ are used to calculate geometry scale consistency loss $L_G$. 
    \item Mask $M_S$ reasons dynamics and occlusions using depth consistency.
    \item Mask $M_a$ from MD2 removes stationary points on image pairs where camera is not moving.
    \item $L = \alpha L^{M}_{P} + \beta L_{S} + \gamma L_{G}$ , where $L^{M}_{P}$ is $L_{P}$ (photometric) weighted by $M_S$. $L_S$ is smoothness loss. Loss is averaged over valid points as decided using $M_a$.
    \item $L_P = sum over V(\lambda * |I_a - I^{'}_{a}| + (1 - \lambda)(1 - SSIM) )$
\end{itemize}

\subsection{Wong Targeted Monocular Depth Adversarial Attack}
